WideSA: A High Array Utilization Mapping Scheme for Uniform Recurrences on the Versal ACAP Architecture

The Versal Adaptive Compute Acceleration Platform (ACAP) is a new architecture that combines AI Engines (AIEs) with reconfigurable fabric. This architecture offers significant acceleration potential for uniform recurrences in various domains, such as deep learning, high-performance computation, and signal processing. However, efficiently mapping these computations onto the Versal ACAP architecture while achieving high utilization of AIEs poses a challenge. To address this issue, we propose a mapping scheme called \fname, which aims to accelerate uniform recurrences on the Versal ACAP architecture by leveraging the features of both the hardware and the computations. Considering the array architecture of AIEs, our approach utilizes space-time transformations based on the polyhedral model to generate legally optimized systolic array mappings. Concurrently, we have developed a routing-aware PLIO assignment algorithm tailored for communication on the AIE array, and the algorithm aims at successful compilation while maximizing array utilization. Furthermore, we introduce an automatic mapping framework. This framework is designed to generate the corresponding executable code for uniform recurrences, which encompasses the AIE kernel program, programmable logic bitstreams, and the host program. The experimental results validate the effectiveness of our mapping scheme. Specifically, when applying our scheme to matrix multiplication computations on the VCK5000 board, we achieve a throughput of 4.15TOPS on float data type, which is 1.11$\times$ higher compared to the state-of-the-art accelerator on the Versal ACAP architecture.

==> draft.tex <==
Motivation:
1. The utilization of AIE array is low in the existing works (64\% for Vitis-AI, 50\% for Vitis-library...)
2. Higher utilization of AIE array leads to difficulty of placement and routing of AIE.

Contribution:
1. Systolic mapping scheme for high utilization.
2. Heuristic routing algorithm for quick and efficient routing.
3. Full-stack framework for mapping.


Outline
1. Abstract
2. Intro
    Utilization of AIE array on Versal ACAP.
    Challenges of achieving high utilization.
    Features of systolic mapping
    Routing algorithm
    contribution
3. Background
    Versal ACAP programming model and workflow
    Systolic design generation
    Motivation
4. Method
    Polyhedral model based two level mapping
    Heuristic routing algorithm
5. Framework
    Mapping, Optimization, Generation
6. Experiments
    1. Setup
    2. Full System Performance
    3. Scalability
    4. Routing success rate
7. Conclusion
